Search-Based Testing of Reinforcement Learning

Evaluation of deep reinforcement learning (RL) is inherently challenging. Especially the opaqueness of learned policies and the stochastic nature of both agents and environments make testing the behavior of deep RL agents difficult. We present a search-based testing framework that enables a wide range of novel analysis capabilities for evaluating the safety and performance of deep RL agents. For safety testing, our framework utilizes a search algorithm that searches for a reference trace that solves the RL task. The backtracking states of the search, called boundary states, pose safety-critical situations. We create safety test-suites that evaluate how well the RL agent escapes safety-critical situations near these boundary states. For robust performance testing, we create a diverse set of traces via fuzz testing. These fuzz traces are used to bring the agent into a wide variety of potentially unknown states from which the average performance of the agent is compared to the average performance of the fuzz traces. We apply our search-based testing approach on RL for Nintendo's Super Mario Bros.

==> Testing of Reinforcement Learning_arxiv/evaluation.tex <==
\pgfplotsset{every tick label/.append style={font=\scriptsize},
label style={font=\scriptsize},
tick label style={font=\scriptsize},
legend style={font=\scriptsize},
legend image code/.code={
\draw[mark repeat=2,mark phase=2]
plot coordinates {
(0cm,0cm)
(0.15cm,0cm)        %% default is (0.3cm,0cm)
(0.3cm,0cm)         %% default is (0.6cm,0cm)
};%
}
}


\section{Experimental Evaluation}
\label{sec:experiments}
We evaluate our testing framework on trained deep RL agents 
for the video game Super Mario Bros., trained 
with varying numbers of training episodes and different
action sets. 

\noindent
\textbf{Setup for RL.} %Due to our focus on testing, 
We use a third-party
RL agent that operates in the OpenAI gym environment and 
uses double deep Q-Networks~\cite{deep_rl_agent}. Details on the learning parameters along with more experiments and the source code are included in the technical appendix.
To evaluate different agents, we test agents at 
varying stages of learning having three different action sets: 
(1) {\em 2-moves:} fast running and jumping to the right. (2)
{\em basic:}  2-moves plus slow running to the right and left.
(3) {\em right-complex:} basic without running left, but actions for pressing up and down, resulting in the largest action set.
%\begin{compactitem}
%    \item {\em 2-moves:} fast running and jumping to the right
%    \item {\em basic:}  2-moves with additional fast running and slow running to the left
%    \item {\em right-complex:} basic moves without running left, but actions for pressing down and up 
%\end{compactitem}
Unless otherwise noted, we present results from training for 
$80k$ episodes. \response{We stopped training at this point since we observed only little improvement from $40k$ to $80k$ episodes, which is also twice as long as suggested~\cite{deep_rl_agent}.}

\noindent
\textbf{Setup for Search and Fuzzing.}
The search for the reference traces uses 
the \emph{2-moves} actions, \response{which are sufficient to
complete most levels in Super Mario Bros. } 
We compute fuzz traces for each action set of the 
different RL agents. We fuzzed for $50$ generations with a population of $50$, used a 
mutation stop-probability $p_{mstop} = 0.2$ with
effect size $ms = 15$ and fitness weights
$\lambda_{cov} = 2$, $\lambda_{pos} = 1.5$, and $\lambda_{neg} = 1$, to focus on exploration.
With a crossover probability of $0.25$, we mostly rely 
on mutations. The search and fuzzing were performed in 
a standard laptop in a few minutes and a few hours, respectively. Compared
to the training that took several days on a dedicated cluster, the computational
effort for testing is relatively low. 
For safety testing, we use $10$ repetitions and a test length of $l=40$
and for performance testing we use $n_{test} = n_{ep} = 10$ and step width $w = 20$.

% \begin{figure}[tb]
%     \centering
% \input{pics/safety_testing_bar_chart}
% \vspace{-0.3cm}
%     \caption{Safety Testing: Relative frequency of fail verdicts. }
%     \label{fig:safety_testing}
% \end{figure}

% \begin{figure}[tb]
%     \centering
%     \input{pics/robust_performance_testing}
% \vspace{-0.6cm}
%     \caption{Robust Performance Testing: Average return of fuzz traces and
%     the 3 agents trained for $20k$ episodes and for $80k$ episodes.}
%     \label{fig:robust_performance_testing}
% \end{figure}

% \begin{figure}[tb]
%     \centering
%     \input{pics/safety_testing_right_complex_detailed}
% \vspace{-0.3cm}
%     \caption{Safety Testing of the \emph{right-complex} agent: Relative frequencies of fail verdicts at boundary states.}
%     \label{fig:safety_testing_detailed_right_complex}
% \end{figure}

% \begin{figure}[tb]
%     \centering
%     \input{pics/safety_vs_reward}
% \vspace{-0.3cm}
%     \caption{Average frequency of safety violations (fails verdicts) and average return during testing with the simple test suite.}
%     \label{fig:safety_vs_reward}
% \end{figure}
\noindent

\noindent

\begin{figure}[t]
	\addtocounter{subfigure}{2}
	\centering
% 	
	\subfloat[Safety Testing: Relative frequency of fail verdicts]{\input{pics/safety_testing_bar_chart}\label{fig:safety_testing}}\\
	\vspace{0.3cm}
	\subfloat[Safety Testing of the \emph{right-complex} agent: Relative frequencies of fail verdicts at boundary states]{\input{pics/safety_testing_right_complex_detailed}\label{fig:safety_testing_detailed_right_complex}}
	\vspace{-0.2cm}
\end{figure}

\begin{figure}[t]
	\addtocounter{subfigure}{4}
	\centering
	\subfloat[Robust Performance Testing: Average accumulated rewards of fuzz traces and
	the agents trained for $20k$ and $80k$ episodes.]{\input{pics/robust_performance_testing} \label{fig:robust_performance_testing}}
	\vspace{-0.2cm}
	\subfloat[Average frequency of safety violations and average accumulated rewards during testing with the simple test suite.]{\input{pics/safety_vs_reward}\label{fig:safety_vs_reward}}\\
	\vspace{-0.2cm}
\end{figure}


\textbf{Safety Testing.}
%\noindent
%\textbf{\RQone}
Fig.~\subref{fig:safety_testing} shows the relative number 
of fail verdicts averaged over all tests at all boundary states for agents with different action sets.
For any agent, all test suites found safety violations. 
For instance, the simple test suite produces fail 
verdicts in about $38\%$ of the cases 
when testing the \emph{right-complex} RL agent.
The agent with 2-moves is tested to be the safest agent, failing only $10\%$ of test cases
of the simple test suite.
For  \emph{right-complex}, the least safe agent,
Fig.~\subref{fig:safety_testing_detailed_right_complex} 
depicts
the relative number of fail verdicts distributed over the boundary states, when 
executing all test suites. Note that the results are affected by stochasticity
and they are normalized, so that all results are within $[0,1]$ even though the 
extended test suites perform more tests.
%All of them include the simple 
%test suite, thus 
%the absolute number of fails is lowest for simple test
%suite in most cases (which is affected by stochasticity), 
%even though its relative fail frequency may be higher. 
We can see that the early boundary states that are explored 
the most cause the least issues.
Furthermore, we observe that the boundary interval
test suite %with $e=1$ 
finds safety violations not detected by the simple test suite, e.g.,
at the boundary states $3$ and $4$. %The agent could not escape safety-critical situations
%from the environment of these states even though the environment is farther from
%unsafe behavior.




% This could result from the fact that fewer training's episodes 
% have reached this boundary state and the agent's behavior is therefore worse.
%This means that in these situations the agent could not escape a safety critical situation from a point farther away from the unsafe behavior.
%The action coverage
%test suites are more thorough by design and point to potential 
%additional unsafe behavior, e.g., close to boundary state $8$.

\noindent
%\textbf{\RQtwo}
\textbf{Robust Performance Testing.}
We perform robust performance testing 
on all agents trained for $20k$ and $80k$ episodes, respectively.
Fig.~\subref{fig:robust_performance_testing} shows the average 
accumulated rewards (y-axis)
gained by the agents and the fuzz traces when performing fuzz trace
prefixes of the length given by the x-axis. 
%The data point at a prefix 
%length of $0$ actually correspond to performance testing via Algorithm~\ref{alg:simple_performance_testing}.
It can be seen 
that initially only the well-trained \emph{2-moves} agent surpasses the performance
benchmark set by the fuzz traces. 
Training for $20k$ episodes is not enough for any agent to
achieve rewards close to the fuzz traces and the 
% \emph{2-moves} agent
% trained for $80k$ episodes comes close and even exceeds the return of the
% fuzz traces, while the 
\emph{basic} agent does not improve much with more 
training.
Hence, a larger action space may hurt robustness. The ability 
to move left of the \emph{basic} agent also increases the state space of the underlying MDP, since only moving right induces a DAG-like structure. 
This explains the poor performance of the \emph{basic} agents. 
%While the \emph{2-moves} agent performs
%better than the fuzz traces in some cases, it performs worse for prefix lengths
%of $40$ and $60$, suggesting that the agent is not robust in states reached
%by fuzz trace prefixes of these lengths.


\noindent\textbf{Relationship between Safety and Performance.}
Finally, we investigate whether performance expressed via 
rewards implies safety. 
Fig.~\subref{fig:safety_vs_reward} shows the average 
number of safety violations % (fail verdicts)
and the average accumulated rewards gained during testing with 
a simple test suite with all
agents trained for $20k$ and $80k$ episodes, respectively.
Comparing the agents with low amount of training,
the safest agent (\emph{basic}) 
is also the one that gains the lowest reward. 
For well-trained agents, 
the safest agent (\emph{2-moves}) also receives the most reward.
%However,
%also in the case of training for $80k$ episodes, \emph{basic} receives
%less reward than \emph{right-complex} despite being safer. 
% There is no positive correlation 
% between safety and reward.
The large negative reward assigned to safety violations
(losing a life) may not be sufficient to enforce safe behavior 
of \emph{right-complex}.
Hence, our testing method may point to issues in reward function design.
However, computing the Pearson correlation coefficient between fail 
verdict frequency and mean accumulated reward for all agents at 
four stages of training with all test suites reveals a moderate negative correlation of $-0.7$, thus high reward often implies low fail frequency.

%, it should be
%taken with a grain of salt, because we have only $48$ data points, which are
%to some extent correlated by design, e.g., results from the same agent, but
%different test suites. 



==> Testing of Reinforcement Learning_arxiv/fuzzTraces.tex <==
Our testing framework evaluates the performance of RL agents
using fuzz traces. The traces are used to
compare gained rewards as well as to bring the agent in a variety of states and to evaluate the performance from these onward. 
In this section, we discuss %a population of 
the fuzz-trace generation for performance testing.
%OLD
%We implement a form of search-based fuzzing~\cite{fuzzingbook2020:02_Lexical_Fuzzing} based on 
%genetic algorithms,
%where we evolve a population of action traces. The search aims to (1) cover a large potion
%of the agent's state space
%(as in pure mutation-based fuzzing~\cite{fuzzingbook2020:02_Lexical_Fuzzing}), 
%while (2) accomplishing the goal specified for RL task. Initializing the trace population
%with the \emph{reference action trace} $\tau_{\mathrm{ref}}$ that already solves the RL task 
%enables an efficient search, with main goal of generating a diverse set of \emph{fuzzed traces}. 
%NEW
% To compute such traces, % a population of traces, 
For this purpose, we propose a search-based 
fuzzing method~\cite{fuzzingbook2021} based on 
genetic algorithms. The goal % of the search 
is to find action traces that (1) cover a large portion
of the state space
%(as in pure mutation-based fuzzing), 
while (2) accomplishing the task to be learned by the RL agent. 


\noindent\textbf{Overview of Computation of Fuzz Traces.}
%OLD
%Initializing the trace population
%with the \emph{reference action trace} $\tau_{\mathrm{ref}}$ %that already solves the RL task 
%enables an efficient search, with main goal of generating a diverse set of \emph{fuzzed traces}.
%NEW
Given the reference trace $\tau_{\mathrm{ref}}$  that solves the RL task (i.e., $s_n \in \states[G]$) and 
parameter values for the number of generations $g$ and the population size $p$, 
%and a
%$k$ determining how many individuals are carried over from one generation to the next (truncation selection), 
the \emph{fuzz traces} are %can be
computed as follows:
\begin{compactenum}
    \item Initialize $\traces_0$, the trace population:%the reference action-trace:
    $~\traces_0 \coloneqq  \{\tau_{\Act, \mathrm{ref}}\}$.
    \item For $i = 1\textbf{ to } g$ generations do:
    \begin{compactenum}
    \item Create $p$ action traces (called \emph{offspring}) from $\traces_{i-1}$ to yield a new population $\traces_i$ of size $p$ by:
        \begin{compactitem}
            \item \emph{either} \emph{mutating} a single parent trace from $\traces_{i-1}$,
            \item  \emph{or} through
        \emph{crossover} of two parents from $\traces_{i-1}$ with a specified crossover probability.
        \end{compactitem}
        \item Evaluate the \emph{fitness} of every offspring trace in $\traces_i$. 
    \end{compactenum}
    % \item Return two sets of traces: $\traces_\mathit{fit}$, containing the fittest trace of each generation,
    % and $\traces_{success}\subseteq \traces_\mathit{fit}$, containing the fittest traces that solve the RL task (end in a state in $\states[G]$).
    \item Return $\traces_\mathit{fit}$ containing the fittest trace of each generation
\end{compactenum}

The \emph{fitness} of a trace is defined in terms of
state-space coverage and 
the degree to which the RL task is solved.
The computation of the fuzz traces searches
iteratively for traces with a high fitness by choosing parent traces with a probability proportional 
to their fitness.
To promote diversity, we favor mutation over crossover, by setting
the crossover probability to a value $<0.5$.
The set of the fittest traces $\traces_\mathit{fit}$ will be used in 
Step 4 for performance testing. Using the single fittest trace
from every generation helps enforcing variety.

\noindent\textbf{Fitness Computation.}
We propose a fitness function especially suited for testing RL agents. For an action trace $\tau_{\Act}$,
%we define 
the fitness $F(\tau_{\Act})$ is the weighted sum
of three normalized terms:
\begin{compactitem}
    \item The \emph{positive-reward term}  $r_{pos}(\tau_{\Act}, s_0)$
    is the normalized positive reward gained in $exec_\tau(\tau_{\Act}, s_0)$. %\todo{by executing it once, right?}
    \item The \emph{negative-reward term} $r_{neg}(\tau_{\Act}, s_0)$ is the 
    normalized inverted negative reward gained in $exec_\tau(\tau_{\Act}, s_0)$.
    \item The \emph{coverage fitness-term} $fc(\tau_{\Act}, s_0)$
    describes the number of newly visited states by
    $exec_\tau(\tau_{\Act}, s_0)$, % It is 
    normalized by dividing
    by the maximum number of newly visited states by any
    action traces in the current population.
\end{compactitem}

\emph{Positive rewards} correspond to the degree as to which the RL task is solved by $\tau_{\Act}$.
\emph{Negative rewards} often correspond to the time required to solve the RL task. Hence if $\tau_{\Act}$ solves the task fast, it would be assigned a small negative reward. We invert the negative reward 
to have only positive fitness terms. 
\response{We normalize $r_{pos}$/$r_{neg}$ by dividing it
by the highest $r_{pos}'$/$r_{neg}'$ in the current generation.} 
%
The \emph{coverage fitness-term} depends on all states visited in previous populations.
Assume that the current generation is $i$. 
Let $Cov_{ppop}$ be the set of all states visited by the previous populations $\bigcup_{j < i} \traces_j$ and let $Cov(\tau_{\Act})$ be the visited states when executing an action trace $\tau_{\Act}$, i.e.,
$Cov(\tau_{\Act}) = \bigcup_{k \leq n}\{s_k\}$,
where $exec_\tau(\tau_{\Act}, s_0) = \langle s_0, a_0, r_0, s_1, \dots, s_n \rangle$.

The \emph{coverage fitness-term} $fc(\tau_{\Act})$ is then given by 
$$fc(\tau_{\Act}) = \frac{|Cov_{ppop} \setminus Cov(\tau_{\Act})|}{\max_{\tau_{\Act}'\in \traces_i}{|Cov_{ppop} \setminus Cov(\tau_{\Act}')|}}.$$ %Thus, 
$fc(\tau_{\Act})$ 
is a normalized value $\leq 1$ and changes during fuzzing as more states are covered.
%This is in line with mutation-based fuzzing in general~\cite{fuzzingbook2020:02_Lexical_Fuzzing}.
The \emph{fitness} $F(\tau_{\Act})$ is given by
$$
F(\tau_{\Act}) = \lambda_{cov} fc(\tau_{\Act}) +
\lambda_{pos} r_{pos}(\tau_{\Act}) + 
\lambda_{neg} (1- |r_{neg}(\tau_{\Act})|), 
$$
where the factors $\lambda_j$ are weights and
$r_{pos}(\tau_{\Act})$ and $r_{neg}(\tau_{\Act})$ are
%positive and negative 
normalized rewards gained when executing $\tau_{\Act}$.

% \noindent
% \textbf{Fitness for our motivating example.}
% In the SMB1 environment, the RL agent receives positive reward for the travelled distance toward the 
% goal post and negative reward for the time spent in the level and for dying, e.g., 
% by falling into a pit. The positive-reward fitness of a trace is the final x-coordinate reached 
% by the agent normalized by the maximal final x-coordinate of all trace in the current population. 
% In order to have only positive fitness terms, we reformulate negative reward into a
% positive property. We compute negative-reward fitness as the relative velocity of Mario controlled
% by an action trace $t$, that is, we divide the final x-coordinate reached by $t$ by the length of
% $t$ and normalize this value using the maximum velocity. We cannot solely use the trace length, 
% because this might encourage creating short traces and we disregard negative reward from dying 
% since this is accounted for in the other fitness components. 



% Assuming we have a \emph{reference action trace} $\tau_{\mathrm{ref}}$,
% that is at the beginning the only trace in our test suite $T$.
% To generate an additional trace to be added to $T$, we perform the following steps:
% \begin{enumerate}
%     \item Pick a trace $\tau\in T$.
%     \item Create \emph{candidate trace} $\tau'$ by applying mutation operators to $\tau$
%     \item Execute candidate trace $\tau'$
%     \item Compare $\tau$ and $\tau'$ and their rewards. If the traces are deemed different enough, according to a certain metric, $\tau$ is added to the test suite $T$. 
% \end{enumerate}

%%%%%%%%%%%%%%%%%%%%OLD%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Mutation \& Crossover.} 
To generate a new action trace,% from existing traces,
we perform either a crossover of two parent traces or
mutate a single parent trace. 
For \emph{crossover}, we create a new offspring trace  splitting two parent traces and concatenating the resulting subtraces. Let $\tau_{\Act,1}$ and $\tau_{\Act,2}$ be the parent action-traces.
To create an offspring trace, we uniformly select a random \emph{crossover point} $i\in\{1,\dots ,\min(|\tau_{\Act,1}|, |\tau_{\Act,2}|)-1\}$. 
%according to a uniform distribution between $1$ and $\min(|\tau_{\Act,1}|, |\tau_{\Act,2}|)-1$. 
The offspring is the concatenation of $\tau^{-i}_{\Act,1}$ and $\tau^{+i}_{\Act,2}$. 
%containing the first $i$ actions of $\tau_{\Act,1}$ and the suffix of $\tau_{\Act,2}$ containing its last $|\tau_{\Act,2}| - i$
%actions. % TODO check off-by-one.
For \emph{mutation}, we repeatedly apply mutation operators.
Given a parent trace $\trace_{\Act}$ and a parameter $ms$
defining the potential effect size of a mutation, we create an offspring $\trace'_{\Act}$ as following:
\begin{compactenum}
    \item Uniformly sample $x\in\{1,\dots,ms\}$.
    \item Chose a mutation operator parametrized with $x$ and perform the mutation on $\trace_{\Act}$ to create an action trace $\trace_{\Act}'$.
    \item Stop with a probability $p_{mstop} \in  (0,1]$ and return %the final offspring trace 
    $\trace_{\Act}'$. Otherwise, set $\trace_{\Act}\leftarrow \trace_{\Act}'$ and continue with Step 1.
\end{compactenum}

%After each such application, we 
%stop with a probability $p_{mstop} \in  (0,1]$ defining the %mutation strength. The possible mutations
%performed on action trace $\tau_{\Act}$ are given by the following list of operators. They are 
%parameterized by $ms$ defining the potential effect size of a mutation, where the 
%actual effect size $as$ is randomly sampled from a uniform distribution over $\{1, \ldots, ms\}$.

The applied mutation operators are (1) Insert, (2) Remove
(3) Change, and (4) Append. Each performs its eponymous
operation on an action sequence of length $x$ at a randomly
chosen index in the parent trace, except for Append.
% Following, we give a list of suitable mutation operators:
% \begin{compactitem}
%     \item \emph{Remove Actions:}
%     Choose a random $i\in [1, |\tau_{\Act}| - x-1]$ and remove $as$ consecutive actions starting
%     at index $i$.
%     %The new traces generated by this mutation operator are all the traces that can be derived from the original trace by removing a single action.
%     \item \emph{Insert Actions:} 
%     Choose a random $i\in [1, |\tau_{\Act}|-1]$ and a random action $a \in \Act$. Insert a sequence 
%     of $x$ consecutive $a$ actions into $\tau_{\Act}$ at index $i$.
%     % This mutation operator repeats an action in the trace. The new traces generated by this mutation operator are all traces, where for every two consecutive actions in the original trace, the first action is repeated.
%     \item \emph{Change Actions:} 
%     Choose a random index $i\in [1, |\tau_{\Act}| - x-1]$ and a random action $a \in \Act$. Replace
%     the subtrace starting at index $i$ of length $x$ with a trace consisting of $x$ consecutive $a$ actions.
%     \item \emph{Append Actions:} 
%     Choose a random action $a \in \Act$ and append $x$ consecutive $a$ actions
%     to $\tau_{\Act}$.% This mutation operator is only applied when %the parent trace of
%     %$\tau_{\Act}$ without appended actions does not reach a terminal state in the execution.
%     % This mutation operator swaps the execution order of two consecutive user actions. The new traces generated by this mutation operator are all traces derived from the original traces where every pair of consecutive actions are swapped
% \end{compactitem}

% \textbf{Comparison metrics.}
% The metrics used to assess if a generated candidate trace $\tau'$ is different enough from $\tau$ to be part of the final test suite $T$ are based on (1) the resulting reward of the execution of $\tau'$ and (2) the trace itself.  We compare two traces based on an adaption of the \emph{Levenshtein distance}. The Levenshtein distance is a string metric which measures the difference between two strings. 
% \textbf{Evaluation of Traces.}
% The goal of fuzzing to create a diverse set of traces from the seed trace created through a 
% deterministic search. We measure variability by computing the average \emph{Levenshtein distance} 
% of all pairs of generated traces. This distance represents the minimum number of single-character edits (insertions, deletions, or substitutions) to transform one word into the other. We
% compare the average Levenshtein distance of fuzz-testing traces to the average distance 
% of traces executed by a trained RL agent executing a randomized policy. 
% This serves to show that the fuzz-testing traces achieve a comparable 
% or large degree of variability, rather than following an action sequence similar to the seed trace. 

% We compute the \emph{average cumulative reward} gained by controlling the agent with 
% fuzz-testing traces. This provides an estimation of what a well-trained RL agent
% with a randomized policy can achieve. 

% We consider two traces to be too similar, if the Levenshtein distance is lower or equal than a specified upper value $\gamma$: $$Levenshtein(\tau_1, \tau_2)\leq \gamma$$. 

% Traces $\tau$ that are too similar to $\tau$ according to their achieved reward and Levenshtein distance are discarded from the final test suite.
% Throwing away a candidate trace means that such candidate was testing behavior already tested by an existing trace.


\begin{algorithm}[t!]
\algorithmfontsize
    \caption{Performance Testing with Fuzz Traces}\label{alg:simple_performance_testing}
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetNoFillComment
    \Input{$\MdpInit$, policy $\pi$, fuzz traces $\traces_\mathit{fit}$,
 \# episodes $n_{ep}$}
    \Output{Avg. accumulated rewards of the agent $R_a$ and the fuzz traces $R_t$}
    \Return $R_t \gets $ \texttt{EvalTraces}($\traces_\mathit{fit}$, $s_0$, $n_{ep}$), 
    $R_a \gets $ \texttt{EvalAgent}($\pi$, $s_0$, $n_{ep}$)\;
    % \Return $R_t,R_a$\;
    
    %\tcc{compute averaged return of trace}
    \SetKwProg{Fn}{Function}{:}{}
    \SetKwFunction{EvalTraces}{EvalTraces}
    \Fn{\EvalTraces{$\traces_\mathit{fit}$, $s_0$, $n_{ep}$}}{
    
    \For{$\tau_{\Act}\in \traces_\mathit{fit}$}{
    \For{$i\gets1$ \text{\normalfont\bf\ to } $n_{ep}$}{
    $\tau_i \gets exec_{\trace}(\tau_{\Act}, s_0) = \langle s_0, a_1, r_1 \dots s_n\rangle$\;
    $R_{t,\tau_{\Act},i}\gets\Sigma^{n}_{k=1} r_k$ with $r_k \in \tau_i$
    }
    }
    \Return $R_t = (\Sigma_{\tau_{\Act}\in \traces_\mathit{fit}}\Sigma_{i=1}^{n_{ep}} R_{t,\tau_{\Act},i}) / (n_{ep} \cdot |\traces_\mathit{fit}|)$
    }
    %\tcc{compute averaged return of agent}
    \SetKwProg{Fn}{Function}{:}{}
    \SetKwFunction{EvalAgent}{EvalAgent}
    \Fn{\EvalAgent{$\pi$, $s_0$, $n_{ep}$}}{
    \For{$i\gets0$ \text{\normalfont\bf\ to } $n_{ep}$}{
    $\tau_i \gets exec_{\pi}(\pi, s_0) = \langle s_0, a_1, r_1 \dots s_n\rangle$ with $s_n\in \states[T]$\;
    $R_{a,i}\gets\Sigma^{n}_{k=1} r_k$ with $r_k \in \tau_i$\;
    }
    \Return $R_a = (\Sigma_{i=1}^{n_{ep}} R_{a,i}) / n_{ep}$
    }
\end{algorithm}

==> Testing of Reinforcement Learning_arxiv/intro.tex <==


In reinforcement learning (RL)~\cite{DBLP:books/lib/SuttonB98}, an agent aims 
to maximize the total amount of reward through trial-and-error via interactions with
an unknown environment. Recently, RL algorithms
achieved stunning results in playing video games and complex board games~\cite{DBLP:journals/corr/abs-1911-08265}.

To achieve a broad acceptance %a wider field of applications 
and enlarge the application areas
of learned controllers, there is the urgent need to reliably evaluate trained RL agents.
When evaluating trained agents, two fundamental questions
% that
need to be answered:
% the following
 \RQone ~\RQtwo
%
Testing deep RL agents is notoriously difficult. %he lack of determinism, combined with the incredible byzantine complexity of the agent's and environmental model and few theoretical guarantees,  makes any kind of testing non-trivial.
%
The first challenge arises from the environment, which is
%considered as complex black-box with
is often not fully known and has
an immense state space,
combined with the byzantine complexity of the agent's model, and the lack of determinism of both the agent and the environment.
Secondly, to evaluate the performance of a trained agent's policy, an estimation of the performance of the optimal policy is needed. %Considering the relation 
%between performance and safety raises a third question: \RQthree\todo{MT:added this here}

To address these challenges, we transfer well-established search-based concepts from software testing into the RL-setting. \emph{Search algorithms} like backtracking-based depth-first search (DFS) are standard  to find valid and invalid program executions. %or satisfying variable assignments in propositional formulas (DPLL ref).
\emph{Fuzz testing} refers to automated software 
testing techniques that generate interesting test cases with the goal to expose corner cases that have not been properly dealt with in the program under test. 
%
In this work, we propose a search-based testing framework to reliably evaluate trained RL agents to answer the questions Q1 and Q2.
Our testing framework comprises four steps:

\noindent \textbf{Step 1: Search for reference trace and
boundary states.}
In the first step, we use a DFS algorithm to search for a \emph{reference trace} that solves the RL task by sampling the black-box environment. 
% This idea is motivated by the intuition that finding a single solution to perform the RL task, while not requiring an optimal solution with respect
% to reward
% %that is not required to be the optimal solution with respect to gained reward, 
% is often computationally very fast.\todo{Sell this better}
This idea is motivated by the experience from AI %game solving
competitions, 
like the Mario AI and the NetHack Challenges \cite{Karakovskiy2012,kuettler2020nethack}, 
where best performers are symbolic agents, 
providing a reference solution of the task 
faster than neural-based agents.
Furthermore, since the DFS algorithm backtracks
when reaching an unsafe state in the environment, 
the search reveals safety-critical situations that we call \emph{boundary states}.
% \todo{Shorten this paragraph one line}

\noindent \textbf{Step 2: Testing for safety.}
To answer Q1, our testing framework computes \emph{safety test-suites}
that bring the agent into safety-critical situations near the boundary states.
Based on the ability of the agent to succeed in
these safety-critical situations we can evaluate the safety of agents.
\response{A safe agent should not 
violate safety regardless of the situation it faces.}

\noindent \textbf{Step 3: Generation of fuzz traces.}
As a basis for performance testing, our testing framework  applies a \emph{search-based fuzzing
method} to compute a diverse set of traces from the reference trace (Step 1) aiming for traces that gain high rewards and cover large parts of the state space.

\noindent \textbf{Step 4: Testing for performance.}
To answer Q2, we  %our testing framework uses 
 create \emph{performance test-suites} from the fuzz traces to bring the agent into a diverse set of states within the environment. As performance metric we propose to point-wise 
compare the averaged performance gained by executing the agent's policy with the averaged performance gained by executing the fuzz traces.

\response{Our approach is very general and can be adapted to 
several application areas. In settings where initial traces are given, for example, stemming from demonstrations by humans, such traces can be used as a basis for fuzzing. Our approach only needs to be able to sample the environment as an oracle. Even in the case of partial observability, our testing framework can be successfully applied. This is the case since we only need the information on whether a trace successfully completed the task to be learned,
partially completed the task, or whether it violated safety.
Exact state information is not required. 
Fuzzing has been applied to test complex software systems, like operating system kernels, 
communication protocols, and parsers for programming lanuages~\cite{DBLP:journals/tse/ManesHHCESW21}. Hence, it offers 
scalability to large environments.
}


In our case study, we apply our framework to test the safety and performance of a set of deep RL agents trained to play Super Mario Bros. Fig.~\ref{fig:mario}
shows the reference trace (red) and boundary states (white points) computed in Step 1 and the
fuzz traces (yellow) from Step 3, computed in our case study.
\response{Since we consider the environment (as well as the trained agent, where a learned policy may need to break ties) to be probabilistic, we execute every test case a number of times and present the averaged results.}
 
 
\noindent \textbf{Related Work.}
%
% The problem of ensuring safety of learned agents has attracted more and more attention in the formal methods community and a large body of work on runtime monitoring and enforcement of RL
\response{While RL has proven successful in solving many complex tasks~\cite{silver2016mastering} and often outperforms
classical controllers~\cite{kiran2021deep}, safety concerns prevent learned controllers from being widely used in safety-critical applications.
The research on \emph{safe RL} targets to guarantee safety during the training and the execution phase of the RL agent~\cite{garcia2015comprehensive}.
Safe RL has attracted a lot of attention in the formal methods community, culminating in a growing body of work on
the verification of trained 
networks~\cite{DBLP:conf/atva/Ehlers17,Pathak2017VerificationAR,DBLP:conf/uai/CorsiMF21}.
However, all of these approaches suffer from scalability issues and are not yet able to verify industrial-size deep neural networks.
An alternative line of research aims to enforce safe operation of an RL agent during runtime, using techniques from runtime monitoring and enforcement ~\cite{DBLP:conf/aaai/AlshiekhBEKNT18,DBLP:conf/amcc/PrangerKTD0B21}.
These methods typically require a complete and faithful model of the environment dynamics, which is often not available.
While a large amount of work on offline and runtime verification of RL agents exists, studying suitable testing methods for RL has attracted less attention.
}

%Testing and verification of (deep) RL agents in large state spaces has received less attention.
The development of RL algorithms has greatly benefited from benchmark
environments for performance evaluation, including the Arcade Learning Environment~\cite{DBLP:journals/jair/BellemareNVB13}, and OpenAI Gym~\cite{brockman2016openai}, Deepmind Control Suite~\cite{tassa2018deepmind}, to name a few. SafetyGym~\cite{Achiam2019BenchmarkingSE} was especially designed to evaluate the safety of RL algorithms during exploration.
Most work on testing for RL evaluates the aggregate performance by comparing the mean and median scores across tasks.
Recently, testing metrics addressing the statistical uncertainty in such point estimates have been proposed~\cite{DBLP:journals/corr/abs-2108-13264}. 
%
We extend previous work by proposing search-based testing tailored toward (deep) RL. We use search-based methods to automatically create safety-critical test-cases and test cases for robust performance testing.

RL has been proposed for software testing and 
in particular also for fuzz testing~\cite{deep_reinf_fuzzing,DBLP:conf/uss/WangZZQKA21,DBLP:conf/fm/ScottSRMG21,DBLP:journals/corr/abs-1807-07490}.
In contrast, we propose a novel search-based 
testing framework including fuzzing to test RL agents. Fuzzing
has been applied to efficiently solve complex tasks% in large state space
~\cite{DBLP:conf/sp/AschermannSAH20,DBLP:journals/corr/abs-2111-03013}.
%, such as playing Super Mario that we also use to evaluate our framework. 
We
perform a backtracking-based search to efficiently solve the task, while fuzzing 
serves to cover a large portion of the state space. 
%
Related is also the work from Trujillo et al.~\cite{DBLP:conf/icse/TrujilloLEDC20} which analyzes the adequacy of neuron coverage for testing deep RL, whereas
our adequacy criteria are inspired by traditional boundary value and combinatorial testing. 

%NEW
\response{
We used our testing framework to evaluate trained deep-Q learning agents, 
agents that internally use deep neural networks to approximate the Q-function.
Recent years have seen a surge in works on testing deep neural networks. 
Techniques, like DeepTest~\cite{DBLP:conf/icse/TianPJR18}, DeepXplore~\cite{DBLP:journals/cacm/PeiCYJ19}, and DeepRoad~\cite{DBLP:conf/kbse/ZhangZZ0K18}, are orthogonal to our proposed 
framework. While we focus on the stateful reactive nature of RL agents, viewing 
them as a whole, these techniques are used to test sensor-related aspects of autonomous agents and find applications in particular
in image processing.
Furthermore, we may consider taking into account neural-network-specific testing
criteria~\cite{DBLP:conf/kbse/MaJZSXLCSLLZW18}. However, doubts about the 
adequacy of neuron coverage and related criteria have been raised recently~\cite{DBLP:conf/sigsoft/Harel-CanadaWGG20}. Hence, more research
is necessary in this area, as has been pointed out by Trujillo et al.~\cite{DBLP:conf/icse/TrujilloLEDC20}.}%, who studied deep RL.}


\noindent \textbf{Outline.} The remainder of the paper is structured as follows.
In Sec.~\ref{sec:prelim}, we give the background and notation. In the Sec.~\ref{sec:searchAlgo} 
to~\ref{sec:performance} 
we present and discuss in detail Step 1 - Step 4 of our testing framework.
We present a detailed case study in Sec.~\ref{sec:experiments}.%, and conclude in Section~\ref{sec:conclusion}.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%---KEEPT FOR SAFE KEEPING------%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
RL algorithms are typically evaluated %overall performance 
on point estimates of aggregate performance such as mean and median scores across a diverse suite of tasks.
The recent shift towards challenging and computationally-demanding RL benchmarks 
makes the evaluation on a large number of runs per task prohibitive and led to the practice of evaluating agents only on a small number of runs per task.
Neglecting the resulting uncertainties in the point estimates over a few runs
led to unfair comparisons of existing RL-algorithms as sown in ~\cite{DBLP:journals/corr/abs-2108-13264}.
\fi

==> Testing of Reinforcement Learning_arxiv/macros.tex <==

%%%%%%%   MDPs

\newcommand{\mdp}{\mathcal{M}}
%\newcommand{\Mdp}[1][]{\ensuremath{\mdp{#1}=(S{#1},I{#1},\Act,\pmdp{#1})}}
\newcommand{\MdpTuple}[1][]{\ensuremath{(\states{#1},\sinit{#1},\Act{#1},\pmdp{#1},\rewFunction{#1})}}
\newcommand{\MdpTupleP}[1][]{\ensuremath{(\states'{#1},\sinit{#1},\Act{#1},\pmdp'{#1},\rewFunction'{#1})}}
\newcommand{\MdpInit}[1][]{\ensuremath{\mdp{#1}=\MdpTuple[#1]}}
\newcommand{\MdpInitP}[1][]{\ensuremath{\mdp{#1}'=\MdpTupleP[#1]}}
\newcommand{\MdpTupleR}[1][]{\ensuremath{(S{#1},\sinit{#1},\Act{#1},\pmdp{#1})}}
\newcommand{\MdpInitR}[1][]{\ensuremath{\mdp{#1}=\MdpTupleR[#1]}}



\newcommand{\sinit}{s_0} % initial state of MDP
\newcommand{\states}[1][]{\mathcal{S}_{#1}}
\newcommand{\act}[1][a]{\alpha} % single action of MDP
\newcommand{\Act}{\mathcal{A}}
\newcommand{\pmdp}{\mathcal{P}}
\newcommand{\rewFunction}{\mathcal{{R}}}

\newcommand{\trace}{\tau}
\newcommand{\traces}{\mathcal{T}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Numbers/Intervals%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\e}{\ensuremath{\mathbb{E}}}

\newcommand{\dist}{\ensuremath{\Delta}_Q}
\newcommand{\exec}{\mathit{exec}}


\DeclareMathOperator*{\argmax}{arg\,max}

==> Testing of Reinforcement Learning_arxiv/performance.tex <==



In the final step, % of our framework, 
we evaluate the performance of trained RL agents. % using the %computed populations of
%fuzz action-traces from Step 3. 
The evaluation
%the performance of an agent by
compares the accumulated reward %(cumulative discounted reward per episode) 
gained from applying the agent's policy with the accumulated reward gained by executing fuzzed traces. 
Especially in RL settings where the maximal expected reward is unknown, the rewards
gained by the fuzz traces serve as a benchmark for the agents'
performance. %to which the agent's performance can be compared
%base values to evaluate the 
%Such an estimation of the 
%quality of learned policies is especially helpful when cumulative rewards are hard to interpret directly.
Furthermore, the fuzz traces are used to test the agents' performance from a diverse set of states.

%for robust performance testing by bringing the agent into a diverse set of states.
%The policy of the agent is evaluated from these states onward. 

%We use fuzz traces, i.e., action traces generated by fuzz testing, for two types of performance
%testing: \emph{global} performance testing and \emph{local} performance testing.
%Both types of testing use a function called $\mathit{eval}(s,ep)$ that evaluates
%the RL agent starting from state $s \in S$ by performing $ep$ episodes, i.e., 
%executions from $s$ to a terminal state. The function computes the average 
%cumulative reward gained in the $ep$ episodes.

 

\begin{algorithm}[t!]
\algorithmfontsize
    \caption{Robust Performance Testing}\label{alg:robust_performance_testing}
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetNoFillComment

    \Input{$\MdpInit$, policy $\pi$, fuzz 
    traces $\traces_\mathit{fit}$, \# tests $n_{test}$, 
    %number of 
    \#~episodes $n_{ep}$,
    step width $w$}
    \Output{Avg. accumulated rewards $R_{t}^{pl}$ and $R_{a}^{pl}$} %after fuzz trace prefixes of length $pl$}
    %\tcc{largest prefix length is the minimum trace length}
    %$\textit{minlen} \gets \min_{\trace\in \traces}(|\trace|)$\;
    $\textit{pl} \gets w$\;
    \Repeat{$|\{\tau_\Act \in \traces_\mathit{fit}:|\tau_\Act| \geq \textit{pl}\}| < n_{test}$ \tcp*[h]{too few traces of length $pl$}}{ 
    \For{$i \gets 1 \text{\normalfont\bf\ to } n_{test}$}{
    $\tau_\Act \gets \text{ random action trace } \in \traces_\mathit{fit}$\;
    $\tau^{-pl} \gets exec_{\trace}(\tau_{\Act}^{-pl}, s_0) = \langle s_0 \dots s_{pl}\rangle$\;
     $R^- \gets \Sigma^{pl}_{t=1} r_t$ with $r_t \in \tau^{-pl}$\;
    
    % \tcc{compute averaged return of fuzz trace}    
    $R_{t,i}^{pl} \gets R^- + $\texttt{EvalTraces}($\{\tau^{pl+}_{\Act}\}$, $s_{pl}$, $n_{ep}$)\;  
    
    % \tcc{compute averaged return of agent trace}
    $R_{a,i}^{pl} \gets R^- + $\texttt{EvalAgent}($\pi$, $ s_{pl}$, $n_{ep}$)\;
    % $i = i + 1$\;
    }
    $R_{t}^{pl} \gets (\Sigma_{i=1}^{n_{test}} R_{t,i}^{pl}) / n_{test}$\;
    $R_{a}^{pl} \gets (\Sigma_{i=1}^{n_{test}} R_{a,i}^{pl}) / n_{test}$\;
    
    $\textit{pl} \gets \textit{pl} + w$\;
    } 
    \Return $\bigcup_{pl} \{pl \mapsto R_{t}^{pl}\},\bigcup_{pl} \{pl \mapsto R_{a}^{pl}\}$
    % $\bigcup_{i=1}^{|\traces_{success}|} R_{t,i}$, $\bigcup_{i=1}^{|\traces_{success}|} R_{a,i}$
    %$i = 0$\;
    % \For{$\tau_{\Act}\in \traces_{success}$}{
    
    % \tcc{compute common prefix trace}
    %  $j = \textit{random integer } \in \{1,\ldots, \lfloor\frac{|\tau_{\Act}|}{2}\rfloor\}$\;
    % $\tau^{-j} = exec_{\trace}(\tau_{\Act}^j, s_0) = \langle s_0, a_0, r_0 \dots s_j\rangle$\;
    % $R_{prefix} = \Sigma^{j}_{t=1} \gamma^t r_t$ with $r_t \in \tau^{-j}$$ 

    % \tcc{compute averaged return of fuzz trace}    
    % $R_{t,i} = R_{prefix} + $\texttt{EvalTraces}($\tau^{j+}_{\Act}$, $s_j$, $n_{ep}$)\;  
    
    % \tcc{compute averaged return of agent trace}
    % $R_{a,i} = R_{prefix} + $\texttt{EvalAgent}($\pi$, $ s_j$, $n_{ep}$)\;
    % $i = i + 1$\;
    % }
    % \Return $\bigcup_{i=1}^{|\traces_{success}|} R_{t,i}$, $\bigcup_{i=1}^{|\traces_{success}|} R_{a,i}$
\end{algorithm}
 
 
\noindent\textbf{Performance Testing.}
%
Simple performance testing starts in a fixed initial state and compares the average accumulated reward of the agent with the average accumulated reward resulting from the execution of fuzz traces.
Given the policy $\pi$ of an agent under test, the fuzz traces $\traces_\mathit{fit}$, an initial state $s_0$, and a number of episodes $n_{ep}$, Algo.~\ref{alg:simple_performance_testing} returns the averaged accumulated rewards
of the agent $R_a$ and the fuzz traces $R_t$. 
%We test global performance of an RL agent by determining the average 
%cumulative reward gained from executions in the RL environment and compare it to the average cumulative reward gained
%by fuzz traces. 


%-----------------------------------------------------OLD------------------------
\noindent\textbf{Robust Performance Testing.}
%
Robust performance testing targets checking the robustness of learned policies
in potentially unknown situations.
For this purpose, we use the fuzz traces to bring the agent
into a diverse set of states and apply the policy of the agent from these states onward until a terminal state is reached.
To cover states close to the initial state as well as close to the goal, 
we actually use fuzz trace prefixes of increasing length.
The averaged accumulated rewards of the agent traces and the fuzz traces 
serve as performance metric. 

Let $\pi$ be the policy of the RL agent under test, 
$\traces_\mathit{fit}$ be the fuzz traces, 
$s_0$ be an initial state, $w$ be a step width 
%with which we
to increase the fuzz trace prefix-length, and $n_{test}$ and $n_{ep}$ be numbers of 
tests and episodes, Algo.~\ref{alg:robust_performance_testing} implements our robust performance testing approach.
Starting from prefix length $pl=w$, for each $pl$ the amount of executed tests is $n_{test}$.
To do so, we first select 
a random trace (line 4) and execute its prefix of length 
$pl$ to arrive at a state $s_{pl}$. From $s_{pl}$, we compute 
the accumulated reward of the fuzz trace (line 6) and of the 
agent averaged over $n_{ep}$ episodes (line 8) and add 
the accumulated reward of the common prefix $R^-$ to both.
We average the accumulated rewards over all tests for each
$pl$ individiually (lines 9 and 10) and finally return all results in Line 13.
% For every action trace $\tau_{\Act} \in \traces_{success}$, we execute the $\tau_{\Act}$ until a random index $j$
% resulting in the state $s_j$. Starting from $s_j$, we compute (1) the averaged return of $\tau^{j+}_{\Act}$, i.e., the suffix of the fuzzed trace $\tau_{\Act}$ from index $j$, and (2) the averaged return of the agent's policy $\pi$ starting from $s_j$.


%The averaged returns are computed with the same functions as in Algo.~\ref{alg:simple_performance_testing}.

%
%\texttt{EvalTraces} : $\mathcal{P}(\mathcal{T}_{\Act}) \times \states \times \N \rightarrow \mathbb{R}$ and \texttt{EvalAgent} : $\Pi \times \states \times \N \rightarrow \mathbb{R}$ as in Algorithm~\ref{alg:simple_performance_testing}. 
 % of the agent $R_a$ and the fuzzed trace $R_t$.
%As performance metric, we compute the ratio of the resulted returns, i.e., $R_{t,pl}/R_{a,pl}$ for every $pl$.


% \iffalse
% \paragraph{Robust Performance Testing.}
% Local performance testing targets checking the robustness of learned policies
% in potentially unknown situations, where the cumulative reward serves as performance metric. 
% For this purpose, we evaluate an RL agent starting from a known state $s_a$ and
% potentially unknown state $s_f$, while ensuring that 
% the distance from the initial state to $s_a$ is approximately the same
% as for $s_f$
% % the distance from $s_a$ 
% % to a goal state approximately matches the distance from $s_f$ to a goal state. 

% Let $\pi$ be the policy of the RL agent under test, 
% let $n_{test}$ be the number of tests, let $n_{ep}$ be the number of
% episodes performed for each test, let
% $\mathcal{T}$ be a set containing $n_{test}$ action traces 
% resulting from executing $\pi$ in the RL environment.  
% Algorithm~\ref{alg:local_performance_testing} implements a single 
% local performance test, i.e., we invoke it once for each trace in $\mathcal{T}$.

% \begin{algorithm}[t!]
%     \caption{Local Performance Testing with Fuzz Traces}\label{alg:local_performance_testing}
%     \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetNoFillComment
%     \Input{MDP $\MdpInit$, an agent trace $at \in \mathcal{T}$, set of fuzz action traces $\mathcal{F}$}
%     \Output{average cumulative reward after: (1) agent trace prefix, $r_a$,
%     fuzz trace prefix $r_f$}
%     $i \gets \textit{random integer } \in \{1,\ldots, \lfloor\frac{|at|}{2}\rfloor\}$ \\
%     $\trace \gets \exec(at^i)$ \tcc{execute random agent prefix} 
%     $\mathit{s_a} \gets \mathit{state}(\trace[i])$ \tcc{final state reached after $\trace$} 
%     $ft \gets \underset{f \in \mathcal{F}}{\argmax}(\dist( \alpha(\mathit{state}(\exec(f^i))),\alpha(\mathit{s_a})))$
%     \tcc{determine fuzz trace prefix}
%     $\mathit{s_f} \gets \mathit{state}(\exec(ft^i))$ \\
%     $\mathit{r_a} \gets \mathit{eval}(\mathit{s_a},n_{ep})$ 
%     \tcc{evaluate from agent trace}
%     $\mathit{r_f} \gets \mathit{eval}(\mathit{s_f},n_{ep})$
%     \tcc{evaluate from fuzz trace}
%     \Return $r_a,r_f$
% \end{algorithm}

% Local performance testing first selects a prefix of random length of a previously
% executed trace. After that it determines the reached abstract state 
% $\mathit{s_a}$ and 
% select a fuzz trace prefix of the same length, such that 
% the distance travelled by RL agent is approximately the same.
% \todo{it is actually more 
% complicated than that, but it is already complicated enough as is \ldots}
% At the same time, the fuzz trace is chosen to reach a states 
% that is as far away from $\mathit{s_a}$ as possible.
% Then, we evaluate the RL agent starting from $\mathit{s_a}$ and from the state
% reached by the fuzz trace prefix. If the RL agent is robust, it should achieve
% a similarly large reward in both evaluate. Hence, we say that a local performance
% test fails if $r_a - r_f > t$ for a testing threshold $t$, i.e., performing
% the fuzz trace leading to an unknown state causes a large drop in reward. 
% Since testing with a single trace $at \in \mathcal{T}$ may not be meaningful, 
% we compute average $r_a - r_f$ resulting from executing Algorithm~\ref{alg:local_performance_testing} for all $at$.

% \noindent
% \textbf{Local Performance Testing of SMB1.}
% Domain knowledge may help to adjust the length of fuzz trace prefixes in order
% to make the testing fairer. In the SMB1 environment, we compute the
% distance $d$ from $\alpha(s_a)$ to a goal state and choose the length 
% of each fuzz trace prefix such that the distance between 
% $\alpha(s_f)$ and the goal is approximately equal to $d$. 
% This is possible in SMB1 as we determine the global x-coordinate of the 
% Mario avatar as part of the part the abstraction $\alpha$ and the 
% goal post is generally at a fixed x-coordinate.
% \fi

==> Testing of Reinforcement Learning_arxiv/safety_testing.tex <==


Based on $\tau_{\mathrm{ref}}$ and $\states[BO]'$ searched for in Step 1, we propose several \emph{test suites} to identify weak points of a policy with a high frequency of fail verdicts, i.e., safety violations.
%We define first a simple boundary test-suite to bring the agent to the boundary-states. 
%Furthermore, we propose two extended test suits to enable a more distinguished analysis by combining the simple test suite with boundary environments and (combinatorial) action coverage.
After discussing suitable test suites, we discuss how to execute them to test the safety of RL agents.


\paragraph{Simple Boundary Test Suite.}
We use the boundary states  $\states[BO]'$ in $\tau_{\mathrm{ref}}$ for
% a form of 
boundary value testing~\cite{pezze_young_testing}.% w.r.t.~a safety objective. 
We compute a simple test suite that consists of all prefixes of $\tau_{\mathrm{ref}}$ that end in a boundary state.
From these traces, we use the action traces  
to bring the RL agent into safety-critical situations and to test its behavior regarding safety.

Formally, let $DB$ be the sequence of depths of the boundary states $\states[BO]'$ in $\tau_{\mathrm{ref}}$, i.e., for any $s_{BO}\in \states[BO]' : d(\tau, s_{BO})\in DB$.
Using $DB$, we compute a set of traces $T$ by 
$$T=\{\tau_{\mathrm{ref}}^{-DB[i]} \mid 1 \leq i \leq |DB| \}.$$
%
Omitting states and rewards from the traces in $T$ results 
in a set of action traces that form a \emph{simple boundary test suite} called $ST$.
%that can lead an RL agent to boundary states
We say the action trace $\tau_{\Act,\mathrm{ref}}^{DB[i]}\in ST$
is the test case for the $i$\textsuperscript{th} boundary state in $\states[BO]'$.

\paragraph{Test Suites using Boundary Intervals.}
Boundary value testing checks not only boundary values,
but also inputs slightly off of the boundary~\cite{pezze_young_testing}.
To transfer this concept into RL testing, 
% the setting of testing for RL
we introduce boundary intervals to test at additional states near the boundary.
% Testing with positive offsets corresponds to testing input values slightly 
% outside the specified range, as is commonly done in traditional boundary
% value testing. 

%TODO: Might be changed to explore all states
%around boundary that are not loosing
In contrast to boundary testing of conventional software, our test cases stay in states traversed by $\tau_{\mathrm{ref}}$.
This choice is motivated by the definition of a boundary state: a state with successor states that necessarily lead to an unsafe state.
Bringing the RL agent in such a losing position will not provide additional insight concerning the learned safety objective, since the agent has no other choice than to violate safety. 
However, testing states of $\tau_{\mathrm{ref}}$ within an offset of boundary states provides insights into
how well the RL agent escapes safety-critical situations. 
%
Given a simple test suite $ST$ and an interval-size $is$, we create an 
\emph{interval test suite} $IT(is)$ by 
adding additional test cases to $ST$, such that 
$$IT(is) = \{\tau_{\Act,\mathrm{ref}}^{DB[i] + \mathit{off}} \:|\: \tau_{\Act,\mathrm{ref}}^{DB[i]} \in ST, 
-is \leq \mathit{off} \leq is\},$$ where $\tau_{\Act,\mathrm{ref}}$ is the reference action-trace.
The test case $\tau_{\Act,\mathrm{ref}}^{DB[i] + \mathit{off}}$ tests the agent at boundary
state $i$ with offset $\mathit{off}$. 


\paragraph{Test Suites using Action Coverage.}
Combinatorial testing covers issues resulting from combinations
of input values. We adapt this concept by creating test suites that cover combinations of actions near boundary states, i.e., the test suite evaluates which actions cause unsafe behavior in boundary regions.
%
%Conversely, test results may also point to action that enforce safety,
%suggesting ways to mprove an RL policy.
%
Given the reference action-trace $\tau_{\Act,\mathrm{ref}}$, a simple test suite $ST$, and a $k \geq 1$, we generate a  
\emph{$k$-wise action-coverage} test suite $AC(k)$ by creating $|\Act|^k$
test cases for every test case in $ST$ covering all $k$-wise combinations
of actions at the $k^{th}$ predecessor of a boundary state.
The test suite is given by $$AC(k) = 
\{\tau_{\Act,\mathrm{ref}}^{DB[i] -k} \cdot \mathit{ac} \:|\: \tau_{\Act,\mathrm{ref}}^{DB[i]} \in ST, 
\mathit{ac} \in \Act^k\}.$$



% TODO: check off-by-one errors and settle on where indexes start (0 or 1), here we use one


\paragraph{Test-case Execution \& Verdict.}

To test the behavior of an agent regarding safety, we use a safety test-suite to bring the agent in safety critical situations. % and observing its behavior from these situation onward.
%
A single test-case execution takes an action-trace $\trace_\Act$,
an inital state $s_0$ and a test length $l$ as parameters. 
To test an RL agent using $\trace_\Act$, we first execute $\trace_\Act$,
yielding a trace $exec(\trace_{\Act})=\langle s_0, a_1, r_1, s_1, \dots , a_n, r_n,s_n \rangle$.
A test case $\trace_\Act$ is \emph{invalid} if $exec(\trace_\Act)$ consistently visits a terminal state in $\states[T]$ when executed repeatedly. 

Starting from $s_n$, we pick the next $l$ actions according to the policy of the agent. 
Note that $l$ should be chosen large enough to evaluate the behavior of the agent regarding safety.
Therefore, it should be considerably larger than the shortest path to the next unsafe state in $S_U$.
%
 %to rule out unwanted, i.e., 
%unsafe behaviour following a boundary state and small enough to not overlap 
%with tests of the succeeding boundary states. 
%OLD
%As a rule of thumb, $l$ should be at least
%as large as the longest path $\tau_m$ from any boundary state such $\tau_m$
%does not traverse another boundary state. 
After performing $l$ steps of the agent's policy, we evaluate the test case.
A test can \emph{fail} or \emph{pass}: A test fails, if starting from $s_n$ the agent reaches an unsafe state 
in $\states[U]$ within $l$ steps. Otherwise, the test passes. 

% NOTE: here, we could say that we can benefit from domain knowledge as in Mario, since 
% there we know how many actions it takes to jump a large gap

To execute a test suite $T$, we perform
every test case of $T$ 
$n$ times. %, given the parameter $n$ to define the number of test-case repetitions.
%Given an entire test-suite $T$ and a parameter $t_{rep}$,
%every test case of $T$ is executed $t_{rep}$
%To execute an entire test-suite $T$, we require another parameter $t_{rep}$ defining how often we repeat each test case of $T$. 
During that, 
we compute 
the \emph{relative frequency of fail verdicts} resulting from 
executing each individual test case.
%and the \emph{average step reward} gained from each action chosen according to the RL agent policy.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COPY - SAVED FOR SAVE KEEPING
% \iffalse

% During the DFS for the reference trace, we find several safety violations from which we backtrack towards 
% a goal state. All branching points in the search tree correspond to potentially unsafe states, thus
% we can use them to identify the boundary of a safe region of MDP states. 

% \paragraph{Simple Boundary Test Suites.}
% We use this information for a form of boundary value testing~\cite{pezze_young_testing} w.r.t. a 
% safety specification. That intuition behind is that prefixes of the reference trace ending
% a branching point bring the RL into a boundary state of the safe region. 
% More formally, let $\tau_{\mathrm{ref}}$ be a reference trace and let $BP$ be a sequence of the depths
% of branching points in the search tree for $\tau_{\mathrm{ref}}$. We define a simple safety test suite $ST$ suite over $\tau_{\mathrm{ref}}$ and
% $BP$ as a set of action traces $ST = \{\tau_{\mathrm{ref}}^{BP[i]} \mid 1 \leq i \leq |BP| \}$. We say
% that $\tau_{\mathrm{ref}}^{BP[i]}$ is a test case for the $i$\textsuperscript{th} boundary state.

% \paragraph{test case Execution \& Verdict.}
% The test case execution takes an action trace $\trace_\Act$ and a test length $l$ as parameters. To test an RL agent, we first execute $\trace_\Act$ and then perform $l$
% action according to the strategy of the RL agent. We say that the test \emph{fails} if we reach a terminal non-goal 
% state after performing $\trace_\Act$, i.e., during the control of the RL agent and we say that the 
% test is \emph{invalid} if we reach a terminal state during the execution of $\trace_\Act$. Otherwise, the 
% test \emph{passes}. All tests of simple test suite either fail or pass when the environment is non-stochastic.

% The test length $l$ should be chosen large enough to rule out unwanted, i.e., 
% unsafe behaviour following a boundary state and small enough to not overlap with 
% tests of the succeeding boundary states. As a rule of thumb, $l$ should be at least
% as large as the longest path $\tau_m$ from any boundary state such $\tau_m$
% does not traverse another boundary state. 
% % NOTE: here, we could say that we can benefit from domain knowledge as in Mario, since 
% % there we know how many actions it takes to jump a large gap

% To execute an entire test suite $T$, we require another parameter $t_{rep}$ 
% defining how often we repeat each test case of $T$. During test-suite execution, 
% we compute two main testing metrics: (1) 
% the \emph{relative frequency of fail verdicts} resulting from 
% executing each individual test case
% and the \emph{average step reward} gained from each action 
% chosen according to the RL agent policy.



% \paragraph{Extended Test Suites.}
% Simple test suites enable us to identify weak points of a policy with a high frequency of fail verdicts, i.e., 
% safety violations. We propose two additional extensions of simple test suite to enable a more distinguished analysis.
% For this purpose, we combine simple test suites with boundary intervals and (combinatorial) action coverage.  

% \noindent
% \textbf{Boundary Intervals.}
% Given a simple test suite $ST$ and an interval size $is$, we create an 
% \emph{interval $e$} test suite $IT(is)$ by 
% adding additional test cases to $ST$, such that 
% $IT(is) = \{\tau_{\mathrm{ref}}^{BP[i] + \mathit{off}} | \tau_{\mathrm{ref}}^{BP[i]} \in ST, 
% -is \leq \mathit{off} \leq is\}$, where $\tau_{\mathrm{ref}}$ is the reference trace.
% The test case $\tau_{\mathrm{ref}}^{BP[i] + \mathit{off}}$ tests the RL agent at boundary
% state $i$ with offset $\mathit{off}$. 
% Testing with positive offsets corresponds to testing input values slightly 
% outside the specified range, as is commonly done in traditional boundary
% value testing~\cite{pezze_young_testing}. 
% In contrast to that, however, we actually stay in the safe region traversed by $\tau_{\mathrm{ref}}$.
% This is motivated by the fact that moving into the unsafe region beyond a boundary state
% will not provide additional insights concerning safety. 
% Testing insight the safe region with offsets may provide insights into
% how well the RL agent escapes boundary region. 
% % Remark for analysis: high fail frequencies with negative offsets suggests that the agent
% % does not move away from the boundary/unsafe region, high fail frequencies with positive 
% % offset suggest that the RL agents will move towards the unsafe region even if we move 
% % away from it. 

% \noindent
% \textbf{Action Coverage.}
% Given a simple test suite $ST$ and a $k \geq 1$, we create  
% \emph{$k$-wise action-coverage} test suite $AC(k)$ by creating $|\Act|^k$
% test cases for every test case in $ST$ covering all $k$-wise combinations 
% of actions at every boundary state.
% The test suite is given by $AC(k) = 
% \{\tau_{\mathrm{ref}}^{BP[i] -k} \cdot \mathit{ac} | \tau_{\mathrm{ref}}^{BP[i]} \in ST, 
% \mathit{ac} \in \Act^k\}$, where $\tau_{\mathrm{ref}}$ is the reference trace.
% With action-coverage test suite, we check which action combinations lead to unsafe behavior, 
% thus covering a larger part of the safety-boundary region. Conversely, test results
% may also point to action that enforce safety, suggesting ways to improve an RL policy.


% % TODO: check off-by-one errors and settle on where indexes start (0 or 1), here we use one

% \fi


==> Testing of Reinforcement Learning_arxiv/search.tex <==


The first step of our testing framework is to perform a \emph{search} for a reference trace $\trace_{\mathrm{ref}}$ that performs the tasks to be learned by the RL agent (not necessarily in the optimal way)
and to detect boundary-states $\states[B0]'\subseteq\states[B0]$ along the reference trace.
%Analysing the backtracking points of the computation of $\trace_{\mathrm{ref}}$ yields to a set of boundary-states 
%$\states[B0]'\subseteq\states[B0]$.
%In step 2 of our testing-framework, the boundary-states $\states[B_0]'$ will be used as initial states for
%safety testing an RL-agent. In step 3, $\trace_{ref}$ will be used to generate the fuzz traces which will in following be used for the performance testing of an RL-agent.
%BK Note:
% Hi, safe regions of MDP states might be something to introduce 
% I am writing now about boundary value testing. In testing, this is usually done by identifying boundaries in the spec.
% Here, I would consider a safety spec. and the boundary are states close to the boundary
% I think the boundary states are states on the boundary of the winning region, i.e., states that can leave the winning
% region with a single action
% Another note from Martin: I am saying stuff like "To test an RL agent, 
% we first execute $\trace_\Act$ and then perform $l$ action according to 
% the policy of the RL agent." 
% Do/should we introduce RL agents as a mathematical object?  --> We could also say "the trained model" and then only "model"
%in the following


We propose to compute $\tau_{\mathrm{ref}}$ using a \emph{backtracking-based, depth-first search} (DFS) by sampling the MDP $\mdp$.
For the DFS, we abstract away stochastic behavior of $\mdp$ by exploring all possible 
behaviors in visited states by repeating actions sufficiently often~\cite{DBLP:conf/icgi/KhaliliT14}.
%following an insight from active automata learning~\cite{DBLP:conf/icgi/KhaliliT14}.
%
Assuming that $p=\mathcal{P}(s,a,s')$ is the smallest transition
probability greater $0$ for any $s,s'\in \states$ 
and $a \in \Act$ in $\mdp$, we 
compute the number of repetitions $rep$  required to match a confidence level $c$ via
$rep(c, p) = log(1 - c)/ log(1 - p)$. 
This ensures observing all possible states with
a probability of at least $c$.
% For a non-terminal state $s \in \states$ and an action $a\in\Act$, we define the \emph{confidence parameter} $c$ to be the probability of observing all transitions $\mathcal{P}(s,a,s')>0$ for any $s'\in \states$.

% Given an MDP $\MdpInit$. 
% For a non-terminal state $s \in \states$ and an action $a\in\Act$, we define the \emph{confidence parameter} $c$ to be the probability of observing all transitions $\mathcal{P}(s,a,s')>0$ for any $s'\in \states$.


% \todo{Martin: I think it would make sense to rearrange that so that 
% $p$ comes first like: Assuming that $p$ is the smallest transition 
% probability, we define the number of repetitions $rep(c,p) = \ldots$ so
% so as to ensure that we observe all possible transitions with confidence $c$,
% i.e., the probability of observing all transitions is at least $c$.}

% Let $p=\mathcal{P}(s,a,s')$ be the smallest transition probability greater $0$ for any $s'\in \states$.
% Given $c$ and $p$, we can compute the 
% number of repetitions $rep$  required to match the confidence level $c$ as follows:
% $$rep(c, p) = log(1 - c)/ log(1 - p).$$ 
%
\textbf{Example.} Assume that $p=0.1$ is the smallest probability $>0$ in $\mdp$.
To achieve a confidence level of $90\%$ that the search visited any reachable state, 
the DFS has to perform $rep(0.9, 0.1)= 22$ repetitions of any action in any state. 

\SetKwFor{RepTimes}{repeat}{times}{end}

\begin{algorithm}[t!]
\algorithmfontsize
    \caption{Search for Reference Trace $\tau_{\mathrm{ref}}$}\label{alg:search}
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetNoFillComment
    \Input{MDP $\MdpInit$, repetitions $rep$}
    \Output{$\tau_{\mathrm{ref}}, \:$ $\states[BO]'$ }


    $\mathcal{V_S} \leftarrow [s_0]; \:\:\:
    \mathcal{V_A} \leftarrow [\:]; \:\:\:
    Explored \leftarrow \emptyset;    \:\:\:
    success \gets \textit{false}$\;
        $\tau_{\mathrm{ref}} \leftarrow [s_0];\:\:\: 
    \states[BO]' \leftarrow \emptyset$\;
    
    \texttt{DFS}($s_0$)\;
    \If{$success$}{
    $s_{\mathrm{prev}} \leftarrow s_0$\;
    \For{$i \in 1,\dots, |\mathcal{V_A}|$}{
    $a, \: s \:\leftarrow\: \mathcal{V_A}[i],\: \mathcal{V_S}[i+1]$\;
    \If{$s\notin Explored$}{
    $r \leftarrow \mathcal{R}(s_{\mathrm{prev}},a, s)$\;
    \textbf{Push}$(\tau_{\mathrm{ref}}, \langle a,r,s\rangle)$\;
    $s_{\mathrm{prev}} \leftarrow s$\;
    % \textbf{Push}$(\tau_{\mathrm{ref}}, s)$\;
    \If{$\mathcal{V_S}[i+2] \in Explored$}{ 
    \tcc{\algorithmfontsize next state is a backtracking point} 
    $\states[BO]' \gets \states[BO]'\cup\{ s\}$\;
    }
    }
    }
    }

    \SetKwProg{Fn}{Function}{:}{}
    \SetKwFunction{DFS}{DFS}
    \Fn{\DFS{$s$}}{
    \If{$s\in\states[U]$}{
    $Explored \gets Explored \cup \{s\};\:\: \Return$\;
    }
    % \If{$s \in \mathcal{V}isited\;$}{
    % $ \Return$\;
    % }
    \If{$s\in\states[G]\;$ \textbf{or} $\; success$}{
     $success \gets true$;$\:\: \Return$\;}
    \For{$a \in \Act$}{
    \RepTimes{$rep$}{
    Sample $s'$ from $ \mathcal{P}(s,a)$\;
    \If{$s'\notin \mathcal{V_S}$}{
    \textbf{Push}($\mathcal{V_A}$, $a$) $;\:\:$
    \textbf{Push}($\mathcal{V_S}$, $s$)\;
    \texttt{DFS}($s'$)\;
    }
    }

    }
    \lIf{$\lnot success$}{
    $Explored \gets Explored \cup 
    \{s\}$}
    }
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%  OLD VERSION  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{algorithm}[t!]
%     \caption{Search for Reference Trace $\tau_{ref}$}\label{alg:search}
%     \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetNoFillComment
%     \Input{MDP $\MdpInit$, repetitions $rep$}
%     \Output{$\tau_{ref}$, $\states[BO]'$ }


%     $\mathcal{V}isited \leftarrow [\:]; \:\:\:
%     Explored \leftarrow \emptyset;    \:\:\:
%     success = false$\;
%      $\tau_{\states} \leftarrow [\:];\:\:\: 
%         \tau_{ref} \leftarrow [\:];\:\:\: 
%     \states[BO]' \leftarrow \emptyset$\;
    
%     \texttt{DFS}($s_0$)\;
%     \If{$success$}{
%     \For{$s \in  \mathcal{V}isited$}{
%     \If{$s\notin Explored$}{
%     \tcc{build $\tau_{\states}$ as sequence of states} 
%     \textbf{Push}$(\tau_{\states}, s)$\;
%     \If{$\mathcal{V}isited.\mathrm{next}[s] \in Explored$}{ 
%     \tcc{next state is a backtracking point} 
%     $\states[BO]' \gets \states[BO]'\cup\{ s\}$\;
%     }
%     }
%     }
%     \tcc{$\tau_{ref}$ as sequence of states, actions, rewards} 
%     \For{$s \in  \tau_{\states}$}{ 
%     Sample $(a,r)$ with $ \mathcal{P}(s,a,\tau_{\states}.next[s])>0$ and 
%     $r = \mathcal{R}(s,a,\tau_{\states}.next[s])$\;    
%     \textbf{Push}($\tau_{ref}, (s,a,r)$)\; 
    
%     }
%     }

%     \SetKwProg{Fn}{Function}{:}{}
%     \SetKwFunction{DFS}{DFS}
%     \Fn{\DFS{$s$}}{
%     \If{$s\in\states[U]$}{
%     $Explored \gets Explored \cup \{s\};\:\: \Return$\;
%     }
%     \If{$s \in \mathcal{V}isited\;$}{
%     $ \Return$\;
%     }
%     \If{$s\in\states[G]\;$ \textbf{or} $\; success$}{
%      $success = true$;$\:\: \Return$\;}
%     \textbf{Push}($\mathcal{V}isited$, $s$)\; 
%     \For{$a \in \Act$}{
%     $\mathcal{S}uccessors \gets \emptyset$ \\
%     \For{$i=0$ to $rep$}{
%     $\mathcal{S}uccessors \gets$ Sample $s'$ from $ \mathcal{P}(s,a)$\;
%     }
%     \For{$s' \in \mathcal{S}uccessors$}{
% %    Receive reward $r=\mathcal{R}(s,a,s')$\;
%     \texttt{DFS}($s'$)\;
%     }
%     }
%     \lIf{$\lnot success$}{
%     $Explored \gets Explored \cup 
%     \{s\}$}
%     }
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
\emph{Algorithm~\ref{alg:search}} gives the pseudo code of our search algorithm to compute $\tau_{\mathrm{ref}}\in\traces$ and a set of 
boundary-states $\states[B0]'\subseteq\states[B0]$. 
The list $\mathcal{V_{\states}}$ stores states that have already been visited, and $\mathcal{V_{\Act}}$ 
stores the executed actions leading to the corresponding states in $\mathcal{V_{\states}}$.
%The set of $Explored$ keeps track of the nodes that have been fully explored or are unsafe.
Every time the search visits an unsafe state
the algorithm backtracks. 
A non-terminal state $s$ is added to $Explored$ if the DFS backtracked to $s$ from all successor states. \response{By tracking visited states
in $\mathcal{V_S}$, 
we ensure that we do not explore a state twice along the same trace. That is, we use $\mathcal{V_S}$ to detect cycles.}
When visiting a goal state,
$\textsc{DFS}(s_0)$ terminates successfully.
In this case, $\tau_{\mathrm{ref}}$ is built from
the set of visited states that were not part of a backtracking branch of the search, i.e., $s\in \tau_{\states}$ if $s\in \mathcal{V_{\states}}$ and $s \not\in Explored$, with corresponding actions in $\mathcal{V_{\Act}}$. 
States $s\in \tau_{\mathrm{ref}}$ that have successor states $s'\in Explored$ are boundary states, i.e., $s\in\states[BO]'$.

\textbf{Example.}
Figure~\ref{fig:search_mdp} shows parts of an MDP $\mdp$
that was explored during a run of our search algorithm.
Found unsafe states are marked red.
After visiting $s_{10}\in \states[G]$ (green circle), the search function $\textsc{DFS}(s_0)$ returns with  $\mathcal{V_{\states}}\!=\! [s_0,\dots,s_{10}]$,
$\mathcal{V_{\Act}}\!=\![a,a,b,a,b,b,a,a,b,b]$
and $Explored=\{s_2,s_3,s_4,s_5,s_8,s_9\}$. 
The reference trace (omitting rewards) is
$\tau_{\mathrm{ref}}=\{s_0,a,s_1,b,s_6,a,s_7,b,s_{10}\}$ and
the subset of boundary states is
$\states[BO]'=\{s_1, s_7\}$ (blue circles).

\textbf{Optimizing Search.} 
Proper abstractions of the state space may be used to merge similar states, thereby pruning
the search space and enabling %well as favoring 
to find cycles in the abstract state space via the DFS.
Detecting cycles speeds up the search since the DFS backtracks when finding an edge to an already visited state.
An example for such an abstraction is omitting the execution time in the state space to merge states. 
%\todo[inline]{Filip: I would eliminate this paragraph, it's just saying that you can make your models smaller by getting rid of states that do not give useful information.}



%TODO: detect circles through abstraction
%The agent may perform actions that do not decrease
%the distance toward goal states.
% In our motivating example Mario example, these are movement
% actions that are blocked by an obstacle, such as, a pipe. 
% Similar actions also exist in navigation tasks where obstacles block movement.
%We label the successor states
%of these actions as terminal to optimize the search, as this forces the search
%to backtrack and try a different route. While these new terminal states
%are not necessarily unsafe, they are relevant for testing the agent's ability
%to circumvent obstacles.
\addtocounter{figure}{1}

\begin{figure}
\centering
\includegraphics[width=7.6cm]{pics/example_search.jpg}
    \caption{Run of the Search Algorithm}
    \label{fig:search_mdp}
\end{figure}







% NOTE to Bettina: to speed up search in Super Mario, we define terminal state as states
% that where Mario dies and where Mario runs into a wall. For safety-testing, we can exclude
% the latter. 
% Reason to include the wall states: these states would otherwise only become terminal when
% time runs out, i.e., the search would search for the longest action trace leading to the 
% goal. By including the wall state, we get close to the fastest. 

% store dead states - all paths leading from there
%leading to the dead states end in bad states
